Made-to-measure galaxy modelling utilising absorption line strength data

We enhance the Syer & Tremaine made-to-measure (M2M) particle method of stellar dynamical modelling to model simultaneously both kinematic data and absorption line strength data thus creating a `chemo-M2M' modelling scheme. We apply the enhanced method to four galaxies (NGC 1248, NGC 3838, NGC 4452, NGC 4551) observed using the SAURON integral-field spectrograph as part of the ATLAS3D programme. We are able to reproduce successfully the 2D line strength data achieving mean chi^2 per bin values of ~1 with >95\% of particles having converged weights. Because M2M uses a 3D particle system, we are also able to examine the underlying 3D line strength distributions. The extent to which these distributions are plausible representations of real galaxies requires further consideration. Overall we consider the modelling exercise to be a promising first step in developing a `chemo-M2M' modelling system and in understanding some of the issues to be addressed. Whilst the made-to-measure techniques developed have been applied to absorption line strength data, they are in fact general and may be of value in modelling other aspects of galaxies.

==> Abstract <==
We enhance the Syer & Tremaine made-to-measure (M2M) particle method of 
stellar dynamical modelling to model simultaneously both kinematic data 
and absorption line strength data thus creating a `chemo-M2M' modelling scheme.  
We apply the enhanced method to four galaxies (NGC 1248, NGC 3838, 
NGC 4452, NGC 4551) observed using the SAURON integral-field spectrograph 
as part of the ATLAS3D programme.  We are able to reproduce 
successfully the 2D line strength data achieving mean chi^2 per bin values 
of ~1 with >95\% of particles having converged weights. Because M2M 
uses a 3D particle system, we are also able to examine the underlying 3D line 
strength distributions.  The extent to which these distributions are plausible 
representations of real galaxies requires further consideration.  Overall we 
consider the modelling exercise to be a promising first step in developing 
a `chemo-M2M' modelling system and in understanding some of the issues to be 
addressed.  Whilst the made-to-measure techniques developed have been applied 
to absorption line strength data, they are in fact general and may be of value 
in modelling other aspects of galaxies.

